Constrained Joint Bit and Power Allocation for Multicarrier Systems

This paper proposes a novel low complexity joint bit and power suboptimal allocation algorithm for multicarrier systems operating in fading environments. The algorithm jointly maximizes the throughput and minimizes the transmitted power, while guaranteeing a target bit error rate (BER) per subcarrier and meeting a constraint on the total transmit power. Simulation results are described that illustrate the performance of the proposed scheme and demonstrate its superiority when compared to the algorithm in [4] with similar or reduced computational complexity. Furthermore, the results show that the performance of the proposed suboptimal algorithm approaches that of an optimal exhaustive search with significantly lower computational complexity.

==> intro_old.tex <==
\section{Introduction}

The demand for wireless radio spectrum is growing dramatically with the accelerated advent of new high data rate wireless applications and services. As reported by many jurisdictions, most of the allocated spectrum experiences low spectrum utilization, whereas heavy spectrum utilization occurs in unlicensed bands \cite{fcc2005notice}. Cognitive Radio (CR), first introduced by Mitola in \cite{Mitola1999}, is a promising wireless communication paradigm that is aware of its radio surroundings and adapts intelligently to improve spectrum efficiency. Unlicensed or cognitive users (CUs) seek to \textit{underlay}, \textit{overlay}, or \textit{interweave} their signals with licensed or primary users (PUs) \cite{kolodzy2005cognitive, srinivasa2007cognitive, goldsmith2009breaking}. The underlay approach allows concurrent transmission of PUs and CUs as in ultrawide band (UWB) systems. CUs spread their transmission over a wide bandwidth, hence their interference is below an acceptable noise floor to PUs. The overlay approach also allows concurrent transmission of PUs and CUs with a premise that CUs use part of their power to assist/relay PUs transmission. The interweave approach allows CUs to opportunistically access voids in PUs frequency bands/time slots under the condition that no harmful interference occurs to PUs. In this paper, we focus on the interweave CR systems.

Orthogonal frequency division multiplexing (OFDM) is recognized as an attractive modulation technique for CR due to its flexibility and adaptivity in allocating vacant radio resources among CUs \cite{weiss2004spectrum}. The problem of adaptively changing the power and constellation size per OFDM CU subcarrier to improve CR system performance has spurred more research interests \cite{wang2007power, bansal2008optimal, zhang2008optimal, kang2009optimal, attar2008interference, zhao2010power}. The performance of OFDM-based CR systems is ameliorated by exploiting the fading channel characteristics, i.e. loading subcarriers with higher channel gains with more power or higher constellation size compared to subcarriers in deep fade. 

Most of the published work in the literature \cite{wang2007power, bansal2008optimal, zhang2008optimal, kang2009optimal, attar2008interference, zhao2010power} focus on improving one objective function of the OFDM-based CR systems, i.e., maximizing the throughput or capacity given a total power budget or interference to the PU. In \cite{wang2007power}, Wang \textit{et al.} propose a novel iterative partitioned water-filling power loading algorithm to maximize the capacity, where the CU power budget (constraints on the interference to the PUs is converted to constraints on the CUs transmitted power) and the peak transmission power per CU subcarrier are considered as constraints. Bansal \textit{et al.} in \cite{bansal2008optimal} investigate the optimal power allocation problem in OFDM-based cognitive radio networks to maximize the CU downlink transmission capacity under a threshold interference introduced to PUs. The authors propose two suboptimal loading algorithms that are less complex while achieve near optimal results. In \cite{zhang2008optimal}, Zhang optimizes the CU transmit power to maximize its capacity with constraints on the PU capacity loss and CU average transmit power. Kang \textit{et al.}, in \cite{kang2009optimal}, study the problem of optimal power allocation to maximize the capacity under a constrained average CU transmit power and interference to the PU. Attar \textit{et al.} in \cite{attar2008interference} maximize the total throughput (of both CU and PU) under a constraint of threshold interference to each user. In \cite{zhao2010power}, Zhao \textit{et al.} maximize the throughput of CU while keeping the interference to the PU is below a certain threshold.

To the best knowledge of the authors, no published work in literature addresses the problem of jointly maximizes the OFDM CU throughput and minimizes the OFDM CU total transmit power subject to a constraint on the OFDM CU BER per subcarrier. Maximizing the OFDM CU throughput improves its data rate, while minimizing the transmit power ensures lower interference levels to PUs. In this paper, we propose a low complexity algorithm that requires no iterations for joint bit and power loading subject to a constraint on the OFDM CU BER per subcarrier in the presence of unknown interference. Closed-form expressions for the optimal bit and power distributions are given.

%joint bit and power loading subject to the BER constraint per subcarrier for OFDM CR systems in the presence of interference. In this paper, we propose a low complexity algorithm that requires no iterations, and jointly maximizes the throughput and minimizes the total transmit power, subject to a constraint on the BER per subcarrier in the presence of unknown interference. Closed-form expressions for the optimal bit and power distributions are given. 

The remaining of the paper is organized as follows. Section \ref{sec:opt} introduces the system models and the proposed joint bit and power loading algorithm. Simulation results are presented in Section \ref{sec:sim}, while conclusions are drawn in Section \ref{sec:conc}.  

%Cognitive Radio (CR), first introduced by Mitola in \cite{Mitola1999}, is a promising wireless communication paradigm that is aware of its surroundings and adapts intelligently to improve spectrum utilization efficiency. It enables unlicensed or cognitive users (CUs) to access the spectrum under the condition that no harmful interference occurs to the existing users (PUs). An attractive modulation technique for CR is Orthogonal Frequency Division Multiplexing (OFDM) which is already adopted by many wireless standards, e.g., IEEE 802.11 WLAN, IEEE 802.16 WiMAX, and LTE \cite{mahmoud2009ofdm}. 
%
%In conventional OFDM-based systems, a fixed bit loading is used on all subcarriers. Thus, the total BER is dominated by the subcarriers that have the worst performance. To improve the system's BER, adaptive bit loading can be employed such that the information is redistributed across subcarriers according to the channel state information. Consequently, adaptive bit loading requires accurate channel estimation at the receiver and a reliable feedback channel between the receiver and the transmitter. 
%
%Different adaptive bit loading algorithms are presented in the literature \cite{hughes1988ensemble, de1998optimal, levin2001complete, wyglinski2005bit, fox1966discrete,  sonalkar2000efficient, papandreou2005new, leke1997maximum, campello1999practical, goldsmith1997variable, fischer1996new, kalet1989multitone}. These algorithms can be categorized according to their operation as follows: greedy algorithms \cite{hughes1988ensemble, de1998optimal, levin2001complete, wyglinski2005bit, fox1966discrete,  sonalkar2000efficient, papandreou2005new,leke1997maximum, campello1999practical}, and water-filling based algorithms \cite{goldsmith1997variable, fischer1996new, kalet1989multitone}.
%
%Greedy algorithms show optimal performance by incrementally allocating an integer number of bits at the cost of high complexity. It was first suggested by Hughes-Hartog \cite{hughes1988ensemble} where one bit is added at a time to the subcarrier requiring the smallest additional power to maximize the throughput. Unfortunately, the algorithm requires extensive amount of subcarrier sorting and it converges very slowly. Campello de Souza \cite{de1998optimal} and Levin \cite{levin2001complete} developed a complete and mathematically verifiable algorithm known as "Levin-Campello" that offers significant improvement to the work of Hughes-Hartog. Wyglinski \textit{et al.} \cite{wyglinski2005bit} proposed an incremental bit loading algorithm with uniform power loading to maximize the throughput while guaranteeing a target mean BER. This algorithm achieves nearly the optimal solution given in \cite{fox1966discrete} but with lower complexity.
%
%On the other hand, water-filling based algorithms formulates the adaptive bit loading problem as a constrained optimization problem that can be solved by classical optimization methods \cite{cover2004elements}. These water-filling based algorithms allocates non-integer number of bits to subcarriers in a non-iterative manner. Hence, it compromises performance for lower complexity as it is generally followed by a rounding-off step to allocate an integer number of bits to the transmitted symbols across all subcarriers, thus lowering the overall data rate \cite{wyglinski2005bit}.
%
%In addition, the adaptive bit loading algorithms can also be categorized according to the system performance improvement factors and system constraints as follows: minimizing the average BER while satisfying target throughput or power requirements or both \cite{fischer1996new}, minimizing the transmission power while satisfying target throughput or BER or both \cite{leke1997maximum,campello1999practical}, and maximizing the throughput while satisfying power or BER requirements or both \cite{wyglinski2005bit,sonalkar2000efficient}.
%
%In this paper, we extend a greedy adaptive bit loading algorithm, proposed earlier in \cite{wyglinski2005bit}, that maximizes the average throughput while targeting an average BER given a fixed power per subcarrier, to accommodate the effect of an NB PU interference on the OFDM CU subcarriers. The level of interference depends on how close the CU transmits in frequency when compared to the PU, given a certain interference power. Moreover, we study the effect of imperfect channel estimation on the proposed algorithm.
%
%The remaining of this paper is organized as follows. Section \ref{sec:model} presents the system models. Section \ref{sec:algo} delineates the adaptive bit loading algorithm. Simulation results are presented in Section \ref{sec:sim}. Finally, conclusions are drawn in Section \ref{sec:future}.



==> proposed.tex <==
\section{Proposed Algorithm} \label{sec:proposed}
The proposed algorithm can be formally stated as follows
\floatname{algorithm}{}
\begin {algorithm}
\renewcommand{\thealgorithm}{} 
\caption{\textbf{Proposed Algorithm}}
\begin{algorithmic}[1]
\STATE \textbf{INPUT} Interference power per subcarrier $i$ ($\sigma^2_{u,i}$), the AWGN variance $\sigma^2_n$, channel gain per subcarrier $i$ ($H_i$), target BER per subcarrier $i$ ($\textup{BER}_{th,i}$), and weighting factor $\alpha$.
\FOR{$i$ = 1,...,$N$}
\IF{$C_i \geq - \frac{4}{1.6} \: \frac{\alpha \ln(2)}{1-\alpha} \: \ln(5\:\textup{BER}_{th,i})$}
\STATE $b_i^*$ and $P_i^*$ are given by (\ref{eq:eq10}) and (\ref{eq:eq12}), respectively.
\IF{$b_i^* \geq$ 2}
\STATE - Round $b_i^*$ to the nearest integer.
\STATE - Recalculate $P_i^*$ according to (\ref{eq:BER}).
\ELSE
\STATE - Null the corresponding subcarrier $i$.
\ENDIF
\ELSE
\STATE Null the corresponding subcarrier $i$.
\ENDIF
\ENDFOR
\STATE \textbf{OUTPUT} The optimal $b_i^*$ and $P_i^*$, $i$ = 1,...,$N$.
\end{algorithmic}
\end{algorithm}
